The maximum discrete surface-to-volume ratio of space-filling curve partitions

Space-filling curves (SFCs) are used in high performance computing to distribute a computational domain or its mesh, respectively, amongst different compute units, i.e.~cores or nodes or accelerators. The part of the domain allocated to each compute unit is called a partition. Besides the balancing of the work, the communication cost to exchange data between units determines the quality of a chosen partition. This cost can be approximated by the surface-to-volume ratio of partitions: the volume represents the amount of local work, while the surface represents the amount of data to be transmitted. Empirical evidence suggests that space-filling curves yield advantageous surface-to-volume ratios. Formal proofs are available only for regular grids. We investigate the surface-to-volume ratio of space-filling curve partitions for adaptive grids and derive the maximum surface-to-volume ratio as a function of the number of cells in the partition. In order to prove our main theorem, we construct a new framework for the study of adaptive grids, notably introducing the concepts of a shape and of classified partitions. The new methodological framework yields insight about the SFC-induced partition character even if the grids refine rather aggressively in localised areas: it quantifies the obtained surface-to-volume ratio. This framework thus has the potential to guide the design of better load balancing algorithms on the long term.

==> 06_measures.tex <==
\section{Measures of shapes} 
\label{sec:mu}


For any $M \in \mathbb{N}$, $q \ge 1$, we denote
\[
	[M]_q :=  \begin{cases}
		\frac{q^M}{q - 1} &\text{if } q > 1\\
		M &\text{if } q = 1.
	\end{cases}
\]


\noindent
Let $\classified{Q}$ be the classification of the shape $Q$, with $A(\classified{Q},l,r)$ cells of depth $l$ and class $r$ for all $1 \le l \le \classified{N}$ and $0 \le r \le d$. We then define for all $M \ge \classified{N} = \depth(\classified{Q})$ the \BF{$(c,M)$-measure} of $Q$ as
\[
	\mu(Q, c, M) := \sum_{l=1}^{\classified{N}} \sum_{r = c}^d A(\classified{Q},l,r) \binom{r}{c} \frac{ [M-l]_{k^{d-c}} } { [M]_{k^{d-c}} }.
\]

  For a given SFC $\Phi$, we denote the maximum $(c,M)$-measure over all shapes of partitions of $\Phi$ with depth less than $M$ as $\mu(\Phi, c, M)$. The $\mu$ measure generalises the continuous volume. Indeed, $\mu(Q, 0, M) = \cv(Q)$ for all $M$. Therefore, $\mu(\Phi, 0, M) = 1$ for all $\Phi$.

The main result of this section is determining the asymptotic behaviour of $\mu(\Phi, c, M)$ as the depth $M$ tends to infinity. The rest of the section is devote to its proof.

\begin{theorem} \label{th:mu}
For $0 \le c \le d-1$, $\lim_{M \to \infty} \mu(\Phi, c, M)$ exists and is positive; for $c = d$, $\limsup_{M \to \infty} \frac{\mu(\Phi, d, M)}{M} > 0$.
\end{theorem}


The rest of this section is devoted to the proof of Theorem \ref{th:mu}. 





We introduce the positive constants
\begin{align*}
	F_1 &:= \binom{d}{c} 2^c\\
	F_2 &:= 2k^d \frac{ k^{d-c} } {1 - k^{d-c}}\\
	F_3 &:= \frac{1}{4}\\
	F_4 &:= 2^d k^d.
\end{align*}



\begin{lemma} \label{lem:mu}
For $0 \le c \le d-1$, $F_1 \le \mu(\Phi, c, M) \le F_2$; for $c = d$, $\mu(\Phi, d, M) \le F_4 M$.
\end{lemma}

\begin{proof}
If $Q$ is the shape of a partition and $Q$ has depth $N$, then it contains at most $2k^d$ boxes of depth $1 \le l \le N$. For $c < d$, a cell $q$ of depth $l$ has $\cv(\boundary^c q) = k^{-l(d-c)}$, hence
\begin{align*}
	\mu(Q, c, M) &= \cv(\boundary^c Q)\\
	&\le \sum_{q \in Q} k^{-l(d-c)}\\
	&\le  \sum_{l=1}^N 2k^d k^{-l(d-c)}\\
	&\le 2k^d \frac{ k^{d-c} } {1 - k^{d-c}} = F_2.
\end{align*}
Conversely, if $Q = \{\hypercube\}$, then $\cv(\boundary^c \hypercube) = \binom{d}{c} 2^c$.

For $c = d$, again each cell in $Q$ of depth $l$ contributes to at most $2^d (1 - l/M)$ of the measure, hence
\begin{align*}
	\mu(Q, d, M) &\le \sum_{l=1}^N 2k^d 2^d \left( 1 - \frac{l}{M} \right)\\
	&\le 2^d k^d 2 \left(N - \frac{N(N+1)}{2M} \right)\\
	&\le 2^d k^d M = F_4 M.
\end{align*}
\end{proof}

For $c < d$, the sequence $\mu(\Phi, c, M)$ is positive and bounded. It is also clearly non-decreasing, therefore it converges. For $c=d$, all that is left is to prove that $\mu(\Phi, d, M) = \Omega(M).$



\begin{lemma}
$\mu(\Phi, d, M) \ge F_3 M + o(M)$.
\end{lemma}

\begin{proof}
Consider the following grid $G_M$ of depth $M$ for all $M \ge 2$ even and the corresponding shape $Q_M$. Firstly, $G_2$ is the regular grid of depth $2$, with cells $g_0, \dots, g_{k^{2d}-1}$ sorted according to $\Phi$ and $Q_2 = \{g_0\}$. Then $G_M$ is obtained from $G_{M-2}$ by subdividing the cell $g_{M/2 - 1}$ twice successively; $Q_M = \{ g_0, g_1, \dots, g_{M/2 - 1} \}$. $Q_M$ is a shape which contains $M/2$ cells, where $g_m$ has depth $2m+2$ for all $0 \le m \le M/2-1$. 

\begin{claim} \label{claim:no_parallel_faces}
$D_m := g_0 \cup \dots \cup g_{m-1}$ does not contain two parallel faces of $g_m$. 
\end{claim}

\begin{proof}
Suppose that it is indeed the case, i.e. $x$ and $y$ are two parallel faces of $g_m$, where $x = g_m \cap g_i$ and $y = g_m \cap g_j$ for some $i,j < m$. The cell $g_m$ does not contain two parallel faces of its parent $\parent{g_m}$, thus either $g_i$ or $g_j$ (say $g_j$ without loss) contains a child of $\parent{g_m}$. But in that case, we obtain $g_m \subseteq \parent{g_m} \subseteq \parent{g_j}$, which is the desired contradiction.
\end{proof}


\begin{claim} \label{claim:far_away_vertex}
For every $0 \le m \le M/2 - 1$, either $g_m$ or $g_{m+1}$ contains a cell of class $d$ of depth at most $2m+5$ in $\classified{Q_M}$.
\end{claim}

\begin{proof}
We only need to prove that for every $0 \le m \le M/2 - 1$, either $g_m$ or $g_{m+1}$ contains a vertex (i.e. a $0$-face) at distance at least $k^{-2m-5}$ to every other cell in $Q_M$. 

According to Claim \ref{claim:no_parallel_faces}, $g_m$ shares $r \le d$ faces with $D_m = g_0 \cup \dots \cup g_{m-1}$. For every $0 \le m \le M/2 - 1$, we prove that if $r < d$, then $g_m$ contains a vertex  at distance at least $k^{-2m-3}$ to all the other cells in $Q_M$. If $r < d$, then $g_m$ has at least two vertices which it does not share with cells in $D_m$ (and hence they are at distance at least $k^{-2m-2}$ to cells in $D_m$). Also, the union $E_m = g_{m+1} \cup \dots \cup g_{M/2-1}$ has a bounding box of size $2 k^{-2m-4} \le k^{-2m-3}$. Therefore, $g_m$ has a vertex at distance at least $k^{-2m-2}$ to $D_m$ and at distance at least $k^{-2m-3}$ to $E_m$. 

Now suppose $r=d$. Since $D_m$ does not contain any pair of parallel faces of $g_m$, it must contain exactly the $d$ faces incident to a given vertex $u$ of $g_m$; thus the opposite vertex $v$ of $g_m$ does not belong to $D_m$. Then $v$ is at distance at least $k^{-\depth(g_m)} = k^{-2m-2}$ from $D_m$. If $v \notin E_m$, then it is at distance at least $k^{-\depth(g_{m+1})} = k^{-2m-4}$ from $g_{m+1}$. Since the diameter of $E_{m+1}$ is at most $k^{-2m-4}$, we obtain that $v$ is at distance at least $k^{-2m-3}$ from $E_m = g_{m+1} \cup E_{m+1}$. If $v \in E_m$, then $g_m$ is at distance at least $k^{-2m-3}$ from $D_m$, and hence $D_{m+1}$ contains only one face of $g_{m+1}$, namely $g_m \cap g_{m+1}$; by the first case, we obtain that $g_{m+1}$ contains a vertex at least $k^{-2m-5}$ from $D_{m+1}$ and $E_{m+1}$.
\end{proof}


Now let $M$ be any integer, and $N = M-1$ if $M$ is odd and $N = M-2$ if $M$ is even. By Claim \ref{claim:far_away_vertex}, either $g_m$ or $g_{m+1}$ contains a cell that contributes to $(M-l)/M \ge (M- (2m+5))/M$ to the  $(d,M)$-measure of $Q_N$. Therefore,
\begin{align*}
	\mu(Q_N, d, M) &= \sum_{l=1}^M A(\classified{Q}_N, l,d) \frac{ M-l } { M }\\
	&\ge \sum_{m=0}^{N/2-1} \frac{ M-(2m+5) } { M }\\
	&= \frac{M}{2} - \frac{M^2}{4M} + o(M) = F_3 M + o(M).
\end{align*}
\end{proof}


%\MGCOMM{Todo. 1. Give an example where it does not converge, with $\Gamma_1$ and $\Gamma_2$ (see notes). Not too many details. 2. Conjecture: the limit exists when $\Gamma$ comes from a finite grammar.} 

%Although for $c=d$ we do not always have a limit, we can show that the sequence $\mu(\Phi, d, M)/M$ is well behaved.
%
%\begin{proposition}
%For $c=d$,
%\[
%	\lim_{M \to \infty} \left\{ \frac{ \mu(\Phi, d, M+1) }{ M+1 } - \frac{\mu(\Phi, d, M)}{M} \right\} = 0.
%\]
%\end{proposition}
%
%\begin{proof}
%For $c=d$, we have
%\begin{align*}
%	\frac{\mu(\Phi, d, M+1)}{M+1} &= \frac{1}{M+1} \sum_{l=1}^{M+1} A(\classified{Q}_1,l,d) \left( 1 - \frac{ l } { M+1 } \right)\\
%	&\le \frac{1}{M} \sum_{l=1}^M A(\classified{Q}_1,l,d) \left( 1 - \frac{ l } { M } \right) + o(1)\\
%	&\le \frac{\mu(\Phi, d, M)}{ M } + o(1),\\
%	\frac{\mu(\Phi, d, M+1)}{M+1} &\ge \frac{1}{M+1} \sum_{l=1}^{M+1} A(\classified{Q}_0,l,d) \left( 1 - \frac{ l } { M+1 } \right)\\
%	&\ge \frac{1}{M} \sum_{l=1}^M A(\classified{Q}_0,l,d) \left( 1 - \frac{ l } { M } \right) + o(1)\\
%	&= \frac{\mu(\Phi, d, M)}{ M } + o(1),
%\end{align*}
%where $Q_0$ and $Q_1$ are shapes maximising $\mu(\Phi, c, M)$ and $\mu(\Phi, c, M+1)$, respectively.
%\end{proof}
%
%

